Very Fast Streaming Submodular Function Maximization

Data summarization has become a valuable tool in understanding even terabytes of data. Due to their compelling theoretical properties, submodular functions have been in the focus of summarization algorithms. These algorithms offer worst-case approximations guarantees to the expense of higher computation and memory requirements. However, many practical applications do not fall under this worst-case, but are usually much more well-behaved. In this paper, we propose a new submodular function maximization algorithm called ThreeSieves, which ignores the worst-case, but delivers a good solution in high probability. It selects the most informative items from a data-stream on the fly and maintains a provable performance on a fixed memory budget. In an extensive evaluation, we compare our method against $6$ other methods on $8$ different datasets with and without concept drift. We show that our algorithm outperforms current state-of-the-art algorithms and, at the same time, uses fewer resources. Last, we highlight a real-world use-case of our algorithm for data summarization in gamma-ray astronomy. We make our code publicly available at https://github.com/sbuschjaeger/SubmodularStreamingMaximization.

==> figures/shower.tex <==
% AirShower 
%
% path with root energy 1.0
\draw[blue] (0.000,0.000) -- (0.200,4.200);

%
% path with root energy 0.9791666666666666
\draw[blue] (0.200,4.200) -- (-0.800,5.067);

%
% path with root energy 0.9513888888888888
\draw[blue] (-0.800,5.067) -- (-1.300,7.267);

%
% path with root energy 0.9180555555555555
\draw[blue] (-1.300,7.267) -- (-1.133,8.800);

%
% path with root energy 0.8347222222222221
\draw[blue] (-1.133,8.800) -- (-2.133,9.800);

%
% path with root energy 0.8109126984126983
\draw[blue] (-2.133,9.800) -- (-1.933,10.800);

%
% path with root energy 0.8109126984126983
\draw[blue] (-2.133,9.800) -- (-1.933,10.800);

%
% path with root energy 0.8347222222222221
\draw[blue] (-1.133,8.800) -- (-1.333,9.667);

%
% path with root energy 0.6918650793650793
\draw[blue] (-1.333,9.667) -- (-1.000,10.867);

%
% path with root energy 0.9180555555555555
\draw[blue] (-1.300,7.267) -- (-1.157,8.133);

%
% path with root energy 0.8466269841269841
\draw[blue] (-1.157,8.133) -- (-1.324,9.333);

%
% path with root energy 0.8466269841269841
\draw[blue] (-1.157,8.133) -- (-0.907,9.000);

%
% path with root energy 0.8132936507936508
\draw[blue] (-0.907,9.000) -- (-1.074,13.200);

%
% path with root energy 0.8132936507936508
\draw[blue] (-0.907,9.000) -- (-1.074,10.200);

%
% path with root energy 0.9513888888888888
\draw[blue] (-0.800,5.067) -- (0.200,5.933);

%
% path with root energy 0.7013888888888888
\draw[blue] (0.200,5.933) -- (0.533,6.933);

%
% path with root energy 0.673611111111111
\draw[blue] (0.533,6.933) -- (0.733,7.933);

%
% path with root energy 0.673611111111111
\draw[blue] (0.533,6.933) -- (0.658,9.133);

%
% path with root energy 0.7013888888888888
\draw[blue] (0.200,5.933) -- (-0.133,6.933);

%
% path with root energy 0.6743618618618619
\draw[blue] (-0.133,6.933) -- (-0.467,7.933);

%
% path with root energy 0.650552338052338
\draw[blue] (-0.467,7.933) -- (0.033,9.133);

%
% path with root energy 0.6743618618618619
\draw[blue] (-0.133,6.933) -- (0.200,7.800);

%
% path with root energy 0.6511060479083735
\draw[blue] (0.200,7.800) -- (0.325,9.000);

%
% path with root energy 0.6511060479083735
\draw[blue] (0.200,7.800) -- (0.057,8.667);

%
% path with root energy 0.9791666666666666
\draw[blue] (0.200,4.200) -- (0.533,5.067);

%
% path with root energy 0.9125
\draw[blue] (0.533,5.067) -- (1.533,6.067);

%
% path with root energy 0.8916666666666666
\draw[blue] (1.533,6.067) -- (1.408,7.067);

%
% path with root energy 0.8604166666666666
\draw[blue] (1.408,7.067) -- (1.075,8.600);

%
% path with root energy 0.8395833333333332
\draw[blue] (1.075,8.600) -- (0.075,10.800);

%
% path with root energy 0.8395833333333332
\draw[blue] (1.075,8.600) -- (0.932,9.467);

%
% path with root energy 0.8604166666666666
\draw[blue] (1.408,7.067) -- (1.608,9.267);

%
% path with root energy 0.7604166666666666
\draw[blue] (1.608,9.267) -- (1.275,10.267);

%
% path with root energy 0.7604166666666666
\draw[blue] (1.608,9.267) -- (1.775,10.133);

%
% path with root energy 0.8916666666666666
\draw[blue] (1.533,6.067) -- (1.783,7.067);

%
% path with root energy 0.8712585034013605
\draw[blue] (1.783,7.067) -- (1.950,11.267);

%
% path with root energy 0.8512585034013604
\draw[blue] (1.950,11.267) -- (2.950,12.133);

%
% path with root energy 0.8512585034013604
\draw[blue] (1.950,11.267) -- (2.075,12.800);

%
% path with root energy 0.8712585034013605
\draw[blue] (1.783,7.067) -- (1.950,8.600);

%
% path with root energy 0.8434807256235827
\draw[blue] (1.950,8.600) -- (1.617,9.600);

%
% path with root energy 0.8434807256235827
\draw[blue] (1.950,8.600) -- (1.807,9.600);

%
% path with root energy 0.9125
\draw[blue] (0.533,5.067) -- (0.367,6.600);

%
% path with root energy 0.8291666666666666
\draw[blue] (0.367,6.600) -- (-0.133,7.467);

%
% path with root energy 0.7958333333333333
\draw[blue] (-0.133,7.467) -- (0.367,9.000);

%
% path with root energy 0.7402777777777777
\draw[blue] (0.367,9.000) -- (0.533,13.200);

%
% path with root energy 0.7958333333333333
\draw[blue] (-0.133,7.467) -- (0.867,9.000);

%
% path with root energy 0.7749999999999999
\draw[blue] (0.867,9.000) -- (0.367,13.200);

%
% path with root energy 0.7749999999999999
\draw[blue] (0.867,9.000) -- (1.033,9.867);

%
% path with root energy 0.8291666666666666
\draw[blue] (0.367,6.600) -- (0.167,7.467);

%
% path with root energy 0.807427536231884
\draw[blue] (0.167,7.467) -- (0.367,9.667);

%
% path with root energy 0.807427536231884
\draw[blue] (0.167,7.467) -- (-0.167,9.000);

%
% path with root energy 1.0
% \draw[blue] (0.000,0.000) -- (0.167,1.533);

%
% path with root energy 0.9523809523809523
\draw[blue] (0.167,1.533) -- (0.367,3.733);

%
% path with root energy 0.9107142857142857
\draw[blue] (0.367,3.733) -- (-0.633,5.267);

%
% path with root energy 0.7996031746031746
\draw[blue] (-0.633,5.267) -- (-0.967,6.467);

%
% path with root energy 0.773962148962149
\draw[blue] (-0.967,6.467) -- (0.033,8.667);

%
% path with root energy 0.7151386195503843
\draw[blue] (0.033,8.667) -- (-0.133,12.867);

%
% path with root energy 0.773962148962149
\draw[blue] (-0.967,6.467) -- (-1.110,10.667);

%
% path with root energy 0.673962148962149
\draw[blue] (-1.110,10.667) -- (-1.610,11.867);

%
% path with root energy 0.673962148962149
% \draw[blue] (-1.110,10.667) -- (-1.443,14.867);

%
% path with root energy 0.7996031746031746
\draw[blue] (-0.633,5.267) -- (0.367,6.133);

%
% path with root energy 0.7791950113378685
\draw[blue] (0.367,6.133) -- (-0.633,7.667);

%
% path with root energy 0.7337404658833231
\draw[blue] (-0.633,7.667) -- (-0.776,11.867);

%
% path with root energy 0.7337404658833231
\draw[blue] (-0.633,7.667) -- (-0.776,8.667);

%
% path with root energy 0.7791950113378685
\draw[blue] (0.367,6.133) -- (0.200,7.333);

%
% path with root energy 0.7553854875283447
\draw[blue] (0.200,7.333) -- (0.325,8.867);

%
% path with root energy 0.7553854875283447
\draw[blue] (0.200,7.333) -- (-0.800,9.533);

%
% path with root energy 0.9107142857142857
\draw[blue] (0.367,3.733) -- (0.567,4.600);

%
% path with root energy 0.8863240418118467
\draw[blue] (0.567,4.600) -- (0.900,5.800);

%
% path with root energy 0.8540659772957176
\draw[blue] (0.900,5.800) -- (0.700,8.000);

%
% path with root energy 0.8318437550734954
\draw[blue] (0.700,8.000) -- (0.825,9.533);

%
% path with root energy 0.8318437550734954
\draw[blue] (0.700,8.000) -- (0.900,9.533);

%
% path with root energy 0.8540659772957176
\draw[blue] (0.900,5.800) -- (-0.100,6.800);

%
% path with root energy 0.7429548661846066
\draw[blue] (-0.100,6.800) -- (0.025,8.333);

%
% path with root energy 0.7429548661846066
\draw[blue] (-0.100,6.800) -- (0.025,8.000);

%
% path with root energy 0.8863240418118467
\draw[blue] (0.567,4.600) -- (0.067,6.800);

%
% path with root energy 0.7613240418118467
\draw[blue] (0.067,6.800) -- (0.317,11.000);

%
% path with root energy 0.69465737514518
% \draw[blue] (0.317,11.000) -- (0.483,12.200);

%
% path with root energy 0.69465737514518
\draw[blue] (0.317,11.000) -- (0.567,12.000);

%
% path with root energy 0.7613240418118467
\draw[blue] (0.067,6.800) -- (0.192,7.800);

%
% path with root energy 0.7242870047748096
\draw[blue] (0.192,7.800) -- (0.317,8.667);

%
% path with root energy 0.7242870047748096
\draw[blue] (0.192,7.800) -- (0.067,9.000);

